Discovering Synergistic Drug Combinations for COVID with Biological Bottleneck Models

Drug combinations play an important role in therapeutics due to its better efficacy and reduced toxicity. Recent approaches have applied machine learning to identify synergistic combinations for cancer, but they are not applicable to new diseases with limited combination data. Given that drug synergy is closely tied to biological targets, we propose a \emph{biological bottleneck} model that jointly learns drug-target interaction and synergy. The model consists of two parts: a drug-target interaction and target-disease association module. This design enables the model to \emph{explain} how a biological target affects drug synergy. By utilizing additional biological information, our model achieves 0.78 test AUC in drug synergy prediction using only 90 COVID drug combinations for training. We experimentally tested the model predictions in the U.S. National Center for Advancing Translational Sciences (NCATS) facilities and discovered two novel drug combinations (Remdesivir + Reserpine and Remdesivir + IQ-1S) with strong synergy in vitro.

==> old.tex <==
\section{Experiments}
\label{sec:experiment}

\textbf{SARS-CoV-2 Data } For SARS-CoV-2 infection, we consider three types of biological targets in our target vocabulary $\mathcal{V}=\set{t_1,\cdots,t_m}$:
\begin{itemize}[leftmargin=*,topsep=0pt,itemsep=0pt]
    \item \emph{Viral proteases}: Replication of SARS-CoV-2 virus requires the processing of two polyproteins by two virally encoded proteases: chymotrypsin-like protease (3CLpro) and papain-like protease (PLpro). Inhibitors that block either protease could inhibit viral replication. We have compiled 3CLpro enzymatic activity~\cite{ncats_3clpro} and PLpro inhibition~\cite{reframe_plpro} data made public by NCATS and ReframeDB.
    \item \emph{Viral entry proteins}: SARS-CoV-2 cell entry depends on angiotensin converting enzyme 2 (ACE2)~\cite{hoffmann2020sars}. Inhibiting ACE2 enzyme or the interaction between SARS-CoV-2 and ACE2 could block viral entry. To this end, we utilize ACE2 enzymatic activity~\cite{ncats_ace2} and Spike-ACE2 protein-protein interaction~\cite{ncats_spike_ace2} from NCATS.
    \item \emph{Host proteins}: \citet{gordon2020sars} identified 335 human proteins physically associated with SARS-CoV-2 viral proteins. Inhibitors for these proteins may also hinder viral replication. Among these proteins, we selected 31 proteins that have sufficient amount of drug-target interaction data in the ChEMBL database (i.e., both positive and negative interactions). 
\end{itemize}
The above drug-target interaction data contains around 20K compounds in total. Our training data for SARS-CoV-2 utilizes another two assays:
\begin{itemize}[leftmargin=*,topsep=0pt,itemsep=0pt]
    \item \emph{Single-agent Activity}: We use the NCATS CPE assay in VeroE6 cells~\citep{ncats_cpe}, which contains around 10K compounds and 320 hits with EC50 $\leq 10 \mu$M.
    \item \emph{Drug Combination}: NCATS performed two combination assays in VeroE6 cells, which contain 160 two-drug combinations~\cite{bobrowski2020discovery,ncats_matrix}. \citet{riva2020discovery} also analyzed synergy between Remdesivir and 20 active compounds identified from their high-throughput screen.
\end{itemize}

\textbf{HIV Data } The training data for HIV comes from the following assays:
\begin{itemize}[leftmargin=*,topsep=0pt,itemsep=0pt]
    \item \emph{Drug-target Interaction}: Existing anti-HIV drugs mainly target viral proteins (HIV-1 protease, integrase and reverse transcriptase) or host proteins involved in viral entry (CCR5, CXCR4 and CD4). We compiled DTI data for these six targets from ChEMBL. 
    \item \emph{Single-agent Activity}: NCI conducted an anti-HIV assay~\cite{nci_hiv} with 35K compounds, among which 309 compounds are active (EC50 $\leq 1 \mu$M).
    \item \emph{Drug Combination}: \citet{tan2012systematic} conducted high-throughput screen for HIV drug combinations. The dataset contains 114 two-drug combinations.
\end{itemize}

\textbf{Evaluation Protocol } Since our goal is to predict synergy against SARS-CoV-2, our validation and test set only consist of SARS-CoV-2 combinations.  All the drug-target interaction, single-drug activity and HIV data are used for training only.
Our validation set contains 20 combinations from \citet{riva2020discovery} and test set contains 72 combinations from \citet{bobrowski2020discovery}. The training set contains 90 SARS-CoV-2 combinations from \cite{ncats_matrix}, where we remove combinations that appear in both the training and test set. 

\textbf{Hyperparameters } For DTI module $\phi$, we adopt default hyperparameters from \citet{yang2019analyzing}, with hidden dimension 300 and three message passing iterations. We set the dimension of DTI vector $|\vz|=100$, with 42 real biological targets (SARS-CoV-2 and HIV) and 58 latent targets, so that the number of real and latent targets are roughly equal. We set $\lambda_1=10, \lambda_2=0.1$ for our final model.

\subsection{Results}
To show the effectiveness of different components, we compare with the following baselines:
\begin{itemize}[leftmargin=*,topsep=0pt,itemsep=0pt]
    \item A GCN trained only on SARS-CoV-2 single-agent and combination data ($\lambda_\mathrm{DTI}=0, |\vz|=100$).
    \item +DTI: A GCN trained only on SARS-CoV-2 single-agent, combination as well as drug-target interaction data ($\lambda_\mathrm{DTI}=10, |\vz|=100$).
    \item +MultiD: A GCN trained on both SARS-CoV-2 and HIV data (single-agent + combination), but without drug-target interaction data ($\lambda_\mathrm{DTI}=0, |\vz|=100$).
    \item +All,-latent: A GCN trained on both SARS-CoV-2 and HIV data (single-agent + combination + drug-target interaction), but the latent targets are removed ($\lambda_\mathrm{DTI}=10,|\vz|=42$).
    \item +All: A GCN trained on both SARS-CoV-2 and HIV data (single-agent + combination + drug-target interaction) ($\lambda_\mathrm{DTI}=10,|\vz|=100$).
\end{itemize}
Our results are shown in Figure~\ref{fig:results}. As expected, the GCN baseline performs poorly, with $0.537 \pm 0.075$ AUC. Adding drug-target interaction data (+DTI) improves the AUC to $0.658 \pm 0.079$. Adding HIV data (+MultiD) improves the AUC to $0.706 \pm 0.088$. 
Our final model, trained with both HIV and drug-target interaction (+All), achieves the best AUC of $0.777 \pm 0.066$. This validates the advantage of adding drug-target interaction data and multi-disease training. Note that if we remove the latent targets (+All,-latent), the performance decreases to $0.718 \pm 0.021$. This also shows the importance of using latent targets to complement missing biological information.

\begin{figure}
    \centering
    \includegraphics[width=0.95\textwidth]{figures/results.pdf}
    \caption{\emph{Left}: Results on SARS-CoV-2 combination test set. Our model (+all) outperforms all other baselines. \emph{Right}: Interpretation of latent targets to new biological targets identified by \citet{riva2020discovery}. The blue circles represent latent targets learned by our best model and the red circles represent new biological targets. We draw an edge between a latent target and a biological target if their matching AUROC is higher than 0.7.}
    \label{fig:results}
\end{figure}

\subsection{Latent Target Interpretation}

While the latent targets are trained to represent biological targets, we found that they are predictive of certain SARS-CoV-2 biological targets that are not provided during training. Therefore, we propose to interpret their biological meaning by the following procedure:
\begin{enumerate}[leftmargin=*,topsep=0pt,itemsep=0pt]
    \item Suppose we have a list of real SARS-CoV-2 targets $\mathcal{C}=\set{c_1,\cdots, c_n}$ that are not provided to the model during training (i.e., $\mathcal{V} \cap \mathcal{C}=\emptyset$). Let $\mathcal{D}_{c_j}$ be the drug-target interaction dataset for $c_j$. 
    \item Compute DTI vectors $\vz_{X_1}, \cdots, \vz_{X_n}$ for each compound $X_i \in \mathcal{D}_{c_j}$. For each latent target $k$, compute the AUROC between DTI labels $y_1,\cdots,y_n$ and predicted DTI scores $\vz_{X_1,k}, \cdots, \vz_{X_n,k}$.
    \item Match latent target $k$ to target $c_j$ if the AUROC is higher than threshold $\tau=0.7$. 
\end{enumerate} 
The target set $\mathcal{C}$ contains 34 biological targets reported in \citet{riva2020discovery} that are correlated with SARS-CoV-2 antiviral activity and have drug-target interaction data in the ChEMBL database. These targets are not provided to the model during training. As shown in Figure~\ref{fig:results}, among the 58 latent targets, 27 of them are matched to the antiviral targets in \citet{riva2020discovery} using the above procedure. This shows that our model is capable of capturing additional SARS-CoV-2 targets through single-agent and combination data.
